Self-Supervised Online Learning for Safety-Critical Control using Stereo Vision

With the increasing prevalence of complex vision-based sensing methods for use in obstacle identification and state estimation, characterizing environment-dependent measurement errors has become a difficult and essential part of modern robotics. This paper presents a self-supervised learning approach to safety-critical control. In particular, the uncertainty associated with stereo vision is estimated, and adapted online to new visual environments, wherein this estimate is leveraged in a safety-critical controller in a robust fashion. To this end, we propose an algorithm that exploits the structure of stereo-vision to learn an uncertainty estimate without the need for ground-truth data. We then robustify existing Control Barrier Function-based controllers to provide safety in the presence of this uncertainty estimate. We demonstrate the efficacy of our method on a quadrupedal robot in a variety of environments. When not using our method safety is violated. With offline training alone we observe the robot is safe, but overly-conservative. With our online method the quadruped remains safe and conservatism is reduced.

==> misc.tex <==

For ease of notation let $\gamma(\theta) \triangleq \lmat \cos \theta & \sin \theta \rmat^T $. 
Based on \eqref{eq:safety_nonsmooth}, satisfying the constraint: 
\begin{equation}
    % (\zeta - \rho_i)^\intercal\lmat \cos \theta \\ \sin\theta \rmat v \geq - \alpha (h(\mb{x}))
    (\zeta - \rho_i)^\intercal\gamma(\theta) v \geq - \alpha( h (\mb{x}) ), \quad
    \forall \; i \in I_{\rm a}
    \label{eq:uni_cbf}
\end{equation}
is sufficient to guarantee the safety of the system with respect to three dimensional location of the pixel by Theorem~\ref{thm:nonsmooth} \cite{ames_control_2014}. We note that assuming that the initial condition is safe with respect to all $i \in NumPix$, then the control barrier function constraint is always feasible since $v=0$ is always a valid input for any state in the safe set.

In this case the CBF constraint \eqref{eq:uni_cbf} can be rewritten equivalently as: 
\begin{align}
    % (\zeta - \rho_i)^\intercal\gamma(\theta) v & \geq - \alpha( h (\mb{x}) ) \\ 
    v & \leq - \frac{\alpha(h(\mb{x}))}{(\zeta - \rho_i)^\intercal\gamma(\theta) }
    \triangleq p(\mb{x} , \rho_i), \quad
    \forall \; i \in I_{\rm a}.
    \label{acute}
    % \\
    % v + \frac{\alpha(h(\mb{x}))}{(\zeta - \rho_i)^\intercal\gamma(\theta) } &  \geq 0
    % \label{constraint_noLgh}
\end{align}
Equation \eqref{acute} is a consequence of Assumption \ref{assp:FoV} due to the fact that the projection of any point $(\zeta - \rho_i)$ onto the heading direction is negative since $(\zeta - \rho_i) \in {\rm FoV}$ and the $0 < \delta < \frac{\pi}{2} $ forms a field of view of less than $\pi $ radians centered at the heading angle. Thus \eqref{acute}
% \ref{constraint_noLgh}
is sufficient to guarantee safety with respect to pixel $\rho_i$.
% For ease of notation let $p(\mb{x}, \rho_i) \triangleq - \frac{\alpha(h(\mb{x}))}{(\zeta - \rho_i)^\intercal\gamma(\theta) }  $.
% The nonsmooth composed constraint is then: 
% \begin{equation}
%     v \leq p(\mb{x} , \rho_i) , \quad
%     \forall \; i \in I_{\rm a}.
%     % i \in \mathbb{N} \textrm{ s.t. } h(\mb{x}) = h_i(\mb{x}, \rho_i)
% \end{equation}


